Bug or not Bug? Analysing the Reasons Behind Metamorphic Relation Violations

Metamorphic Testing (MT) is a testing technique that can effectively alleviate the oracle problem. MT uses Metamorphic Relations (MRs) to determine if a test case passes or fails. MRs specify how the outputs should vary in response to specific input changes when executing the System Under Test (SUT). If a particular MR is violated for at least one test input (and its change), there is a high probability that the SUT has a fault. On the other hand, if a particular MR is not violated, it does not guarantee that the SUT is fault free. However, deciding if the MR is being violated due to a bug or because the MR does not hold/fit for particular conditions generated by specific inputs remains a manual task and unexplored. In this paper, we develop a method for refining MRs to offer hints as to whether a violation results from a bug or arises from the MR not being matched to certain test data under specific circumstances. In our initial proof-of-concept, we derive the relevant information from rules using the Association Rule Mining (ARM) technique. In our initial proof-of-concept, we validate our method on a toy example and discuss the lessons learned from our experiments. Our proof-of-concept demonstrates that our method is applicable and that we can provide suggestions that help strengthen the test suite for regression testing purposes.

==> inputsTable.tex <==
\begingroup
\setlength{\tabcolsep}{7pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table}[!ht]
    \centering
    \caption{Combination of the input a and input b}
	\label{tbl:inputs}
    \resizebox{\linewidth}{!} {

    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \diagbox{\textbf{input$_a$}}{\textbf{input$_b$}} & \textbf{0} & \textbf{1} & \textbf{2 }& \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9}  \\ \midrule

        0 & (0,0) & (0,1) & (0,2) & (0,3) & (0,4) & (0,5) & (0,6) & (0,7) & (0,8) & (0,9) \\ \midrule
        1 & (1,0) & (1,1) & (1,2) & (1,3) & (1,4) & (1,5) & (1,6) & (1,7) & (1,8) & (1,9) \\ \midrule
        2 & (2,0) & (2,1) & (2,2) & (2,3) & (2,4) & (2,5) & (2,6) & (2,7) & (2,8) & (2,9) \\ \midrule
        3 & (3,0) & (3,1) & (3,2) & (3,3) & (3,4) & (3,5) & (3,6) & (3,7) & (3,8) & (3,9) \\ \midrule
        4 & (4,0) & (4,1) & (4,2) & (4,3) & (4,4) & (4,5) & (4,6) & (4,7) & (4,8) & (4,9) \\ \midrule
        5 & (5,0) & (5,1) & (5,2) & (5,3) & (5,4) & (5,5) & (5,6) & (5,7) & (5,8) & (5,9) \\ \midrule
        6 & (6,0) & (6,1) & (6,2) & (6,3) & (6,4) & (6,5) & (6,6) & (6,7) & (6,8) & (6,9) \\ \midrule
        7 & (7,0) & (7,1) & (7,2) & (7,3) & (7,4) & (7,5) & (7,6) & (7,7) & (7,8) & (7,9) \\ \midrule
        8 & (8,0) & (8,1) & (8,2) & (8,3) & (8,4) & (8,5) & (8,6) & (8,7) & (8,8) & (8,9) \\ \midrule
        9 & (9,0) & (9,1) & (9,2) & (9,3) & (9,4) & (9,5) & (9,6) & (9,7) & (9,8) & (9,9) \\ \bottomrule
	\end{tabular}}
\end{table}
\endgroup

